A Novel Feature-Based Approach to Characterize Algorithm Performance for the Traveling Salesman Problem

Meta-heuristics are frequently used to tackle NP-hard combinatorial optimization problems. With this paper we contribute to the understanding of the success of 2-opt based local search algorithms for solving the traveling salesman problem (TSP). Although 2-opt is widely used in practice, it is hard to understand its success from a theoretical perspective. We take a statistical approach and examine the features of TSP instances that make the problem either hard or easy to solve. As a measure of problem difficulty for 2-opt we use the approximation ratio that it achieves on a given instance. Our investigations point out important features that make TSP instances hard or easy to be approximated by 2-opt.

==> tbl_earth_model_nrnd.tex <==
% latex table generated in R 2.15.0 by xtable 1.7-0 package
% Tue May 15 12:13:33 2012
\begin{tabular}{lr}
  \toprule
Spline & Coefficient \\ 
  \midrule
(Intercept) & 1.137 \\ 
  h(mst\_dists\_sd-0.0368926) & -2.420 \\ 
  h(0.0368926-mst\_dists\_sd) & 3.733 \\ 
  h(angle\_mean-1.50355) & 0.076 \\ 
  h(1.50355-angle\_mean) & -0.028 \\ 
  h(distance\_max-1.24326) & -0.075 \\ 
  h(1.24326-distance\_max) & -0.115 \\ 
  h(mst\_depth\_mean-17.18) & 0.008 \\ 
  h(17.18-mst\_depth\_mean) & -0.007 \\ 
  h(17.18-mst\_depth\_mean)*h(mst\_dists\_sd-0.0858119) & 0.178 \\ 
  h(17.18-mst\_depth\_mean)*h(0.0858119-mst\_dists\_sd) & -0.116 \\ 
  h(distance\_max-1.24326)*h(mst\_dists\_mean-0.107919) & 2.589 \\ 
  h(distance\_max-1.24326)*h(0.107919-mst\_dists\_mean) & -7.396 \\ 
  h(instance\_size-50)*h(distance\_max-1.24326) & 0.005 \\ 
  h(50-instance\_size)*h(distance\_max-1.24326) & -0.002 \\ 
  h(17.18-mst\_depth\_mean)*h(mst\_dists\_sum-0.0173026) & 0.734 \\ 
  h(17.18-mst\_depth\_mean)*h(0.0173026-mst\_dists\_sum) & -0.062 \\ 
  h(mst\_depth\_sd-10.758) & -0.009 \\ 
  h(10.758-mst\_depth\_sd) & 0.011 \\ 
  h(angle\_mean-1.50355)*h(angle\_sd-1.10555) & -0.514 \\ 
  h(angle\_mean-1.50355)*h(1.10555-angle\_sd) & -0.154 \\ 
  h(angle\_mean-1.50355)*h(angle\_median-1.95446) & -0.032 \\ 
  h(angle\_mean-1.50355)*h(1.95446-angle\_median) & -0.129 \\ 
  h(mst\_dists\_mean-0.115223) & -1.054 \\ 
  h(0.115223-mst\_dists\_mean) & -1.873 \\ 
  h(instance\_size-25) & 0.002 \\ 
  h(chull\_area-0.7604)*h(1.24326-distance\_max) & 1.953 \\ 
  h(0.7604-chull\_area)*h(1.24326-distance\_max) & -0.605 \\ 
  h(angle\_mean-1.74047)*h(10.758-mst\_depth\_sd) & 0.010 \\ 
  h(1.74047-angle\_mean)*h(10.758-mst\_depth\_sd) & 0.004 \\ 
  h(centroid\_min\_distance\_to\_centroid-0.152541)*h(0.115223-mst\_dists\_mean) & 5.821 \\ 
  h(0.152541-centroid\_min\_distance\_to\_centroid)*h(0.115223-mst\_dists\_mean) & -0.343 \\ 
  h(angle\_mean-1.50355)*h(centroid\_centroid\_y-0.5015) & 0.575 \\ 
  h(angle\_mean-1.50355)*h(0.5015-centroid\_centroid\_y) & 0.593 \\ 
  h(mst\_dists\_mean-0.126588)*h(mst\_dists\_sd-0.0368926) & 10.842 \\ 
  h(0.126588-mst\_dists\_mean)*h(mst\_dists\_sd-0.0368926) & 12.913 \\ 
  h(mst\_depth\_median-8)*h(0.0368926-mst\_dists\_sd) & -0.456 \\ 
  h(8-mst\_depth\_median)*h(0.0368926-mst\_dists\_sd) & -0.443 \\ 
  h(instance\_size-25)*h(chull\_points\_on\_hull-0.12) & 0.001 \\ 
  h(instance\_size-25)*h(0.12-chull\_points\_on\_hull) & -0.004 \\ 
  h(angle\_mean-1.50355)*h(nnds\_median-0.23) & 0.272 \\ 
  h(angle\_mean-1.50355)*h(0.23-nnds\_median) & -0.271 \\ 
  h(angle\_mean-1.50355)*h(centroid\_centroid\_x-0.4534) & 0.070 \\ 
  h(angle\_mean-1.50355)*h(0.4534-centroid\_centroid\_x) & 1.361 \\ 
  h(distance\_mean-0.553905)*h(0.0368926-mst\_dists\_sd) & 57.642 \\ 
   \bottomrule
\end{tabular}

